High-Fidelity Audio Generation and Representation Learning with Guided Adversarial Autoencoder

Unsupervised disentangled representation learning from the unlabelled audio data, and high fidelity audio generation have become two linchpins in the machine learning research fields. However, the representation learned from an unsupervised setting does not guarantee its' usability for any downstream task at hand, which can be a wastage of the resources, if the training was conducted for that particular posterior job. Also, during the representation learning, if the model is highly biased towards the downstream task, it losses its generalisation capability which directly benefits the downstream job but the ability to scale it to other related task is lost. Therefore, to fill this gap, we propose a new autoencoder based model named "Guided Adversarial Autoencoder (GAAE)", which can learn both post-task-specific representations and the general representation capturing the factors of variation in the training data leveraging a small percentage of labelled samples; thus, makes it suitable for future related tasks. Furthermore, our proposed model can generate audio with superior quality, which is indistinguishable from the real audio samples. Hence, with the extensive experimental results, we have demonstrated that by harnessing the power of the high-fidelity audio generation, the proposed GAAE model can learn powerful representation from unlabelled dataset leveraging a fewer percentage of labelled data as supervision/guidance.

==> abstract.tex <==




Using "Generative Adversarial Neural Network (GAN)" to generate high fidelity conditional audio samples and learn representation from unlabelled audio data, are two challenging tasks in the field of machine learning research. However, the representation learned from unlabelled data without any supervision does not guarantee its' usability for any downstream task at hand. This would be a wastage of the resources if the training was conducted for that particular downstream task. Also, during the representation learning, if the model is highly biased towards the downstream task, it losses its generalisation capability. This makes the learned representation barely useful for any other tasks that are not related to that downstream task at hand. In this paper, we address this issue by proposing "Guided Adversarial Autoencoder (GAAE)", which can generate superior conditional audio samples from unlabelled audio data using a fewer percentage of labelled data as guidance. Using this superior conditional generation, GAAE can learn representation specific to the downstream task leveraging the guidance from fewer labelled data. Furthermore, GAAE also learns another type of representation capturing the general attributes of the data, which is independent of the downstream task at hand.




% To address this shortcoming, we propose a new autoencoder based model named "Guided Adversarial Autoencoder (GAAE)", which can learn both post-task-specific representations and the general representation capturing the factors of variation in the training data leveraging a small percentage of labelled samples. Furthermore, GAAE can generate audio with superior quality, which is indistinguishable from the real audio samples. 











% Unsupervised disentangled representation learning from the unlabelled audio data, and high fidelity audio generation have become two pillars in machine learning research. However, the representation learned from an unsupervised setting does not guarantee usability for any downstream task at hand. This is a wastage of the resources, if the training was conducted for that posterior job. Also, during the representation learning, if the model is highly biased towards the downstream task, it losses its generalisation capability which directly benefits the downstream job but the ability to scale it to other related task is lost. To address this shortcoming, we propose a new autoencoder based model named "Guided Adversarial Autoencoder (GAAE)", which can learn both post-task-specific representations and the general representation capturing the factors of variation in the training data leveraging a small percentage of labelled samples. Furthermore, GAAE can generate audio with superior quality, which is indistinguishable from the real audio samples. 

% Hence, with the extensive experimental results, we have demonstrated that by harnessing the power of the high-fidelity audio generation, the proposed GAAE model can learn powerful representation from unlabelled dataset leveraging a fewer percentage of labelled data as supervision/guidance.



% Unsupervised disentangled representation learning from the unlabelled audio data and high fidelity audio generation have become two pillars in machine learning research. However, the representation learned from an unsupervised setting does not guarantee its usability for any downstream task at hand. This would be a wastage of the resources if the training was conducted for that posterior task. Also, during the representation learning, if the model is highly biased towards the downstream task, it losses its generalisation capability which directly benefits the downstream job but the ability to scale it to other related task is lost. To address these two shortcomings, we propose a new autoencoder based model named "Guided Adversarial Autoencoder (GAAE)", which can learn two types of representation from unlabelled dataset leveraging a small percentage of labelled samples. In one representation, it targets to learn specific representation according to the provided guidance, which can be used for any related downstream task at hand and in another representation, it learns the general representation capturing the factors of variation in the training data. Furthermore, in this paper, we also aim to generate audio with superior quality. So, the GAAE model is built in a way so that it can also generate high fidelity audio using a few labelled samples. 



% 1 . using adversarial generative networks to learn representation from unlabelled data requires high quality sample generation capability as well as 

==> intro_bkp1_1.tex <==
Learning meaningful representation from the unlabelled dataset is a challenging task \cite{goodfellow_book:2016} but recent advancement of the Generative Adversarial Neural Network (GAN) \cite{goodfellow:2014} has shown great success \cite{donahue2019large, dumoulin2016adversarially, DonahueKD16} in this field. Recent work of Deepmind \cite{donahue2019large} shows that the superior generation power of GAN~\cite{karras:2017, karras2019style, Andrew_biggan} is useful for learning good representation. While the successes of the GAN are based on the image generation tasks, it does not perform well on the audio generation tasks \cite{engel2019gansynth}. Encouragingly, recently some studies \cite{engel2019gansynth,chris_wspecgan,andrTIFGAN} have shown intriguing results in audio generation. This prompts for further studies of these methods to learn representation from unlabelled audio data. Now a days disentangled representation is getting tremendous interest as it offers different factor of variations of any dataset to be easily separable in the representation space \cite{bengio2013representation} which is an indication for a good representation learning \cite{peters2017elements,bengio2013representation,goodfellow_book:2016, Michael05069}. Though some GAN based studies have claimed good result for learning disentangled representation from unlabelled data \cite{radford2015,zhao:2017,chen2016infogan,makhzani:2016,chorowski_wavenet_autoencoder,karras2019style,donahue2019large}, recent work of Google AI has shown both theoretically and practically that unsupervised disentangled representation learning is fundamentally impossible and some form of supervision is necessary to achieve this goal \cite{francesco_2019}. Therefore, for learning a good representation using GANs, it requires good generation as well as some supervision.

\noindent Direct generation of the raw audio waveform is a very complex task. The wavenet generative neural network \cite{waveNet} got some success in raw waveform generation, however, the proposed method was computationally expensive and slow. Rather than using GANs to generate a raw waveform, recent works on generating audio spectrogram (time-frequency representations of audio) and then converting them to audio has shown tremendous success \cite{GANSynth08710, chris_wspecgan,marafioti2019adversarial}. In this process, if the spectrogram can be generated successfully, the next challenge becomes to the conversion of the spectrogram to the audio. In TiFGAN paper \cite{marafioti2019adversarial} using the Phase-gradient heap integration (PGHI) \cite{zden_25} method, authors have shown a minimal loss for audio reconstruction from the spectrogram. Among the GAN architectures, the BigGAN model has performed better in terms of image generation and also in terms of representation learning \cite{Andrew_biggan}. So BigGAN can be used to generate a high-quality spectrogram and representation. Nevertheless, to achieve a better result with BigGAN architecture, we need to provide an enormous amount of data with labels \cite{lucic2019highfidelity}. Though it is easy to find lots of open-sourced datasets, getting labels for them is very expensive. However, the recent work of Deepmind with BigGAN has achieved state of the art (SOTA) generation \cite{lucic2019highfidelity} performance using fewer labels, but the methods discussed in the paper are not suitable for representation learning.

\noindent Representation learning from unlabelled data is ideal so that it can be used for other scenarios where vast labels data is not presented. 
Here we learn representation from one dataset and then use it for another dataset, so the validation of the representation learning can not be conducted after the completion of the first training, making representation learning very difficult. Suppose we have a huge amount of unlabelled audio data of different animal sounds along with daily human-made sounds and a small labeled dataset for classifying x numbers of animal sounds. We assume that these specific animal sounds are presented in the unlabelled dataset. Now we want a model to learn representation from this unlabelled audio data disentangling the animal sound characteristics so that it can be used to learn animal sound classification from the small labeled dataset. But recent work of Google AI \cite{francesco_2019} has claimed that perfect disentangled representation can not be learned from unsupervised methods, so there is no guarantee that this model will disentangle animal sounds in the representation space making it unreliable for post animal sound classification training. It would be useful if we could guide the model to learn post task specific representation so in this paper, we have tried to address this problem through proposing a new GAN architecture where we can guide the GAN model with small labeled data samples to focus on specific characteristics when learning the representation as well as generates superior quality samples. Our contribution in this paper can be summarized as


\begin{itemize}
\item We have proposed a new guided representation learning model named Guided Generative Adversarial Neural Network (GGAN). The sample generation and representation learning capability is justified.  
\item As our model is based on the BigGAN model, we have explored the bigGAN architecture for generating audio spectrograms in both unsupervised and supervised manner, where we have validated the model after converting the spectrogram to audio. The representation learning of the unsupervised BigGAN is explored for audio data.     
\end{itemize}








==> justbackup.tex <==
% %\documentclass[a4paper,12pt]{article}

% \usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
% \usepackage[utf8]{inputenc}
% \usepackage{sectsty}
% \usepackage{titlesec}
% \usepackage{import}
% \title{
% % High-Quality Audio Generation and Representation Learning with Guided Generative Adversarial Neural Network (GGAN) using Fewer Labelled Data
% % / 
% Guided Generative Adversarial Neural Network for Learning Task-specific Representation and Generating High-Quality Audio Sample Leveraging Fewer Labelled Audio Data
% }
% \author{}
% \date{September 2018}
% \setcounter{secnumdepth}{4}
% \usepackage{graphicx}
% \graphicspath{ {images/} }
% % \documentclass[a4paper,12pt]{article}
% % \usepackage[utf8]{inputenc}
% % \usepackage[english]{babel}
% \usepackage{graphicx}
% % \usepackage[round]{natbib}
% % \usepackage[nottoc]{tocbibind} %Adds "References" to the table of contents
% % For algorithms
% \usepackage{algorithm}
% % \usepackage{algorithmic}
% \usepackage{amsmath}
% \usepackage{algcompatible}
% \usepackage{globalThings}
% % \usepackage[utf8]{inputenc}
% % \usepackage{blindtext}
% % \usepackage[utf8]{inputenc}
% % \usepackage{blindtext}
% \usepackage{color}
% % \import{}{front_page.tex}
% % %Document title, author and date (empty)
% % \title{Unsupervised  Disentangled  Representation Learning  from  audio}
% % \author{Kazi Nazmul Haque}
% % \date{}
% % \usepackage{pageslts}
% % \usepackage{fancyhdr}
% % \pagestyle{fancy} 
% % \fancyhf{}
% % \renewcommand{\headrulewidth}{0pt}
% \usepackage{pageslts}
% \usepackage{fancyhdr}
% \pagestyle{fancy} 
% \fancyhf{}
% \renewcommand{\headrulewidth}{0pt}
% \usepackage{setspace}

% \usepackage{xfrac}
% % \usepackage{lineno}
% \usepackage{longtable}


% \begin{document}

% % \doublespacing
% % % \newpage
% % % \renewcommand*\contentsname{Table of Contents}
% % \pagenumbering{roman}
% % \cfoot{\thepage}
% % \tableofcontents
% % \clearpage

% % \pagenumbering{arabic}
% % \cfoot{\thepage}
% % \linenumbers

% \maketitle

% % \begin{abstract}


% % \import{}{abstract.tex}
 




% % \end{abstract}






% % %\section{Introduction}
% % %\import{}{intro.tex}

% % %\section{Background and Related Work}
% % %\import{}{background.tex}


% % %\section{Proposed Research Methods}

% % %\import{}{proposed_method.tex}

% % \section{Data and Implementation Detail}
% % %\import{}{data.tex}

% % \section{Results}
% % %\import{}{results.tex}

% % \section{Conclusion}
% % %\import{}{conclusion.tex}

% % \newpage
% % \medskip
% % \bibliographystyle{acm}
% % \bibliography{references}



% \end{document}








==> proposed_method.tex <==
\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=.6 \linewidth]{GAE_model.jpg}}
    \caption{This figure illustrates the overall architecture of the GAAE model. Different networks of the GAAE model are shown along with the connections between them. In the figure, the arrows are coloured to highlight the flow of any input/output of the model. For the discriminator, the red boxes show the fake samples and the green boxes indicate  the real samples. Here, $x_{u}$ is the unlabelled data sample, $x_{l}$ is the labelled data sample,$\hat{x}_{u}$ is the reconstructed data sample, $y_{r}$ is the random conditions, and $z$ is the known latent distribution.}
    \label{fig:model_architecture}
\end{figure*}


\subsection{Architecture of the GAAE}

The GAAE consists of five neural networks: the Encoder $E$, the Decoder $D$, the Classifier $C$, the Latent Discriminator $L$ and the Sample Discriminator $S$. Let the parameters for these networks be $\theta_{e}$, $\theta_{d}$, $\theta_{c}$, $\theta_{L}$, and $\theta_{S}$ respectively. Figure \ref{fig:model_architecture} shows the whole architecture of the model and the description is as follows. 

\subsubsection{Encoder}

The Encoder $E$ takes any unlabelled data sample $x_{u}$ $\sim$ $p_{data}$ and outputs two latent samples $z_{x_{u}}$ $\sim$ $u_z$ and $z^{'}_{x_{u}}$ $\sim$ $q_z$, where $p_{data}$ is the true unlabelled data distribution, and $u_z$,$q_z$ are two different continuous distributions learned by the $E$. We require the latent $z_{x_{u}}$ to capture the post-task-specific attributes/characteristics  of the data and the latent $z^{'}_{x_{u}}$ to capture the general/style attributes of the data.

\subsubsection{Classifier}

We have a classifier network $C$ which is trained with limited labelled data  $x_{l}$ $\sim$ $p_{ldata}$, where $p_{ldata}$ is the labelled data distribution and not necessarily $p_{ldata}$ $\subset$ $p_{data}$. Here, with this $p_{ldata}$, the whole model gets guidance---thus, we call this data as ``guidance data''. Now, the $C$ network takes any latent sample and predicts the category class for that latent sample. To train $C$, we pass $x_{l}$ through the $E$ network and get two latent vectors \{$z_{x_{l}}$,$z^{'}_{x_{l}}$\} = $E(x_{l};\theta_{e})$. Then, we only forward $z_{x_{l}}$ through $C$ to get the predicted label $\hat{y}_{x_{l}}$ = $C(z_{x_{l}};\theta_{c})$ and train $C$ against the true label $y_{l}$ $\sim$ $Cat(y_{l},k = n)$ of the sample $x_{l}$, where $Cat(y_{l},k = n)$ is the categorical distribution with $n$ numbers of categories/labels. These labels are used as one-hot vector. For now, lets consider that $C$ can classify the label of any sample correctly.

\subsubsection{Decoder}
The Decoder $D$ maps any latent and categorical class/label variable to the data sample. Now, to get the reconstructed sample of $x_{u}$, we pass the latent $z^{'}_{x_{u}}$ and the label of $x_{u}$ through the $D$ network. As $x_{u}$ is an unlabelled data sample, we get the label $\hat{y}_{x_{u}}$ = $C(z_{x_{u}},\theta_{c})$ through the network $C$ and obtain the reconstructed sample $\hat{x}_{u}$ = $D(z^{'}_{x_{u}},\hat{y}_{x_{u}} ; \theta_{d})$ from the $D$ network. 
Here, we also want to use the $D$ network for generating samples according to the given condition along with the reconstruction. Therefore, the same latent $z^{'}_{x_{u}}$ is used with a random categorical variable (one-hot vector) $y_{r}$, sampled from categorical distribution $Cat(y_{r}, K = n,p = \frac{1}{n})$ , where $n$ is the number of categories/labels, and the sampling probability for each category is $\frac{1}{n}$. Now, we obtain the generated sample $\hat{x}_{g}$ $\sim$ $p_{gdata}$, where $p_{gdata}$ is the generated data distribution by the $D$ network, and it is trained to match $p_{gdata}$ with the true data distribution $p_{data}$. Here, the size of $n$ is the same as of the guided data, and we want the $D$ network to generate data according to the categories from the guided data. Therefore, we ensure this with the Discriminator where the Discriminator receives the labels of the data from the network $C$.  
As we use a small number of labelled data, it is hard to train $C$ due to the problem of overfitting. Hence, we use the generated sample $\hat{x}_{g}$ and train the $C$ network considering $y_{r}$ as the true label/category, where the predicted label is $\hat{y}_{\hat{x}_{g}}$ = $C(E(\hat{x}_{g},\theta_{e}),\theta_{c})$. 

Here, $C$ depends on the correct conditional generation from $D$, and $D$ depends on the classification from the network $C$. During the training, the $C$ network starts to predict the category of some samples from the given labelled data correctly. Likewise, the Discriminator learns to identify the correct category for those samples and forces the $D$ network to generate samples with the attributes related to these correctly classified samples. These generated samples bring more characteristics with them, which are not present in the given labelled data but belong to the data distribution. Now, as we feed these generated samples again to the $C$ network with the associated conditional categories as correct labels, it learns to predict the correct category for more samples related to that generated samples. Then again, these new correctly classified samples improve the conditional generation of the $D$ network. Hence, throughout the training, the $C$ network and $D$ network improve each other continuously. Meanwhile, during the training, the representation learning (latent generation) capability of the $E$ network is also ameliorated via the process of reconstructing sample $x_{u}$, which also improves the performance of the $C$ and $D$ network eventually.   

\subsubsection{Discriminators}

The GAAE model has two discriminators: the Sample Discriminator $S$ and the Latent Discriminator $L$. $S$ makes sure that the generated sample $\hat{x_{g}}$ and the reconstructed sample $\hat{x_{u}}$ match the sample from the true data distribution $p_{data}$. We train $S$ with the sample and its label. Now, for the samples $\hat{x_{g}}$ and $\hat{x_{u}}$, we have the labels $y_{r}$,$\hat{y}_{x_{u}}$ respectively. Hence, the pairs  $(\hat{x_{g}},y_{r})$ and $(\hat{x_{u}},\hat{y}_{x_{u}})$ are considered fake labels for the discriminator $S$. For the true data, both $x_{l}$ and $x_{u}$ are used together, where we get the label for the sample $x_{u}$ from $C$, and, for the sample $x_{l}$ we use the available true labels. Hence, in terms of distribution perspective, we obtain the data distribution $p_{mdata}$, mixing the distributions $p_{ldata}$ and $p_{data}$. Accordingly, $S$ is trained with the true sample data $x$ $\sim$ $p_{mdata}$ along with its associated label $y$ if it  exists, otherwise with the predicted label from $C$.

Here, the network $E$ learns to map the general characteristics of the data onto the latent distribution $q_z$, excluding the categories from the guided data. Now, if we can draw the sample from the  $q_z$ distribution, then, by using the categorical distribution as condition, we can generate diverse data for different categories (categories from the guided data) from the Decoder $D$. We can only sample from $q_z$, if the distribution is known to us. Therefore, we use another Discriminator $L$ so that the $E$ network is forced to match $q_z$ to any known distribution $p_z$, where $p_z$ can be any known continuous random distribution (e.\,g.,  Continuous Normal Distribution, or Continuous Uniform Distribution). The $L$ network is trained through differentiating between the true latent $z$ $\sim$ $p_z$ and the fake latent $z{'}_{x_{u}}$.  

\subsection{Losses}


\subsubsection{Encoder, Classifier and Decoder}

For the $E$ and $D$ networks, we have the sample generation loss $G_{loss}$, the sample reconstruction loss $R_{loss}$, and the latent generation loss $L_{loss}$.
To calculate the generation and discrimination loss, we use hinge loss, and for the reconstruction loss the Mean Squared Error (MSE) loss. For the $G_{loss}$, we take the average of the generation loss for $\hat{x_{u}}$ and $\hat{x_{g}}$. Therefore,   

\begin{equation}
\label{eq:1}
\begin{aligned}
G_{loss} = -\frac{1}{2}(S(\hat{x_{u}},\hat{y}_{x_{u}} ; \theta_{s}) + S(\hat{x_{g}},y_{r}); \theta_{s}).\\
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:2}
\begin{aligned}
L_{loss} = -(L( z^{'}_{x_{u}}; \theta_{l}).\\
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:30}
\begin{aligned}
R_{loss} = \frac{1}{N}\sum\limits_{i=1}^N{ (\hat{x}_{u_{i}} - x_{u_{i}})^{2}}.\\
\end{aligned}
\end{equation}

Now, for the $C$ network, we calculate the classification loss $Cl_{loss}$, $Cg_{loss}$ for the labelled data sample $x_{l}$ and the generated sample $\hat{x_{g}}$ respectively. Here, $\hat{x_{g}}$ is used as a constant, so it is considered like a sample data $x_{l}$. We only forward propagate $x_{u}$ through $E$ and $D$ and no gradient is calculated for generating $\hat{x_{g}}$ when it is only used for the loss $Cg_{loss}$. The model is implemented with pytorch \cite{paszke2019pytorch} and we detach the gradient of $x_{g}$ when $Cg_{loss}$ is calculated. Therefore,

\begin{equation}
\label{eq:3}
\begin{aligned}
Cl_{loss} = - \sum y_{l} \log \hat{y}_{x_{l}}.\\
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:4}
\begin{aligned}
Cg_{loss} = - \sum y_{r} \log \hat{y}_{\hat{x}_{g}}.\\
\end{aligned}
\end{equation}

We get the a combined loss $EDC_{loss}$ for $E$,$D$ and $C$. The $EDC_{loss}$ is calculated as 

\begin{equation}
\label{eq:5}
\begin{aligned}
EDC_{loss} = \alpha \cdot (\omega_{1} \cdot G_{loss} + \omega_{2} \cdot ( \lambda \cdot R_{loss})) + 
\\ \beta \cdot (\omega_{3} \cdot Cl_{loss} + \omega_{4} \cdot Cg_{loss} + \omega_{5} \cdot L_{loss}).\\
\end{aligned}
\end{equation}

Here, the weights of the $E$,$C$, and $D$ networks are updated to minimise the loss $EDC_{loss}$, where $\omega_{1}$, $\omega_{2}$, $\omega_{3}$, $\omega_{4}$, $\omega_{5}$, $\alpha$, $\beta$, and $\lambda$ are the hyperparameters. The successful training of our GAEE model depends on these parameters. At the beginning of the training, we noticed that the value of $R_{loss}$ falls rapidly compared to other losses and results in a very small gradient value. To mitigate this problem, we multiply $R_{loss}$ with a hyperparameter $\lambda$ $\in$ $\mathbb{R}_{> 0}$ and after hyperparameter tuning, we found 20 as an optimal value for  $\lambda$. The $D$ network of the model is tuned for both the reconstruction loss $R_loss$ and the generation loss $G_loss$. Therefore, to balance between these two losses, the hyperparameter $\omega_{1}$ and $\omega_{2}$ is used where $\omega_{1}$, $\omega_{2}$ $\in$ $[0,1]$ and $\omega_{1}$ + $\omega_{2}$ = 1. Here, we can force the model to focus more on either loss by increasing the hyperparameter for that particular loss. Likewise, for $Cl_{loss}$, $Cg_{loss}$ and $L_{loss}$, we use the hyperparameters $\omega_{3}$, $\omega_{4}$, $\omega_{5}$ respectively, where  
$\omega_{3}$, $\omega_{4}$, $\omega_{5}$ $\in$ $[0,1]$ and $\omega_{3}$ + $\omega_{4}$ + $\omega_{5}$ = 1. In the $EDC_{loss}$, $G_{loss}$ and $R_{loss}$ are responsible for the sample generation quality, where  $Cl_{loss}$, $Cg_{loss}$ and $L_{loss}$ are responsible for the latent generation quality. So, to balance between sample generation and latent generation, we use two hyperparameters $\alpha$ and $\beta$, where $\alpha$, $\beta$ $\in$ $[0,1]$, and  $\alpha$ + $\beta$ = 1.

\subsubsection{Discriminators' loss}

For the Discriminators $S$ and $L$, we use hinge loss. The discrimination loss for the fake samples are averaged as we calculate the loss for both $\hat{x}_{u}$ and $\hat{x}_{g}$. Let the discrimination loss for $S$ and $L$ be $S_{loss}$, $L_{loss}$ respectively. Therefore, 

\begin{equation}
\label{eq:6}
\begin{aligned}
S_{loss} = - min(0, -1 + S(x, C(E(x,\theta_{e});\theta_{c}) ; \theta_{s})) \\
-  \frac{1}{2} (min(0, -1 - S(\hat{x}_{u}, \hat{y}_{x_{u}}; \theta_{s})) \\+ min(0, -1 - S(\hat{x}_{g}, \hat{y}_{r}; \theta_{s}))). \\
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:7}
\begin{aligned}
L_{loss} = - min(0, -1+ L(z,\theta_{l}) \\- min(0,-1-L(\hat{z}_{x_{u}},\theta_{l})). \\
\end{aligned}
\end{equation}


Here, we update the parameters $\theta_{s}$ and $\theta_{l}$ to maximise the loss  $S_{loss}$ and $L_{loss}$ respectively.  Algorithm 1 shows the training mechanism for the GAAE model. 

\begin{algorithm}[t!]
\caption{\small Minibatch stochastic gradient descent training of the proposed GAAE model. The discriminator is updated $k$ times in one iteration. Here, for our experiment, we use  $k=2$ for better convergence.}

\begin{algorithmic}[1]
\label{alg:AGF1}
\FOR{number of training iterations}
  \FOR{$k$ steps}
    
    \STATE { Sample the latent/noise samples $ \{ \bm{z^{(1)}}\dots, \bm{z^{(m)}} \} $ from $p_z$, the conditions (labels) $ \{ \bm{y_{r}^{(1)}}, \dots, \bm{y_{r}^{(m)}} \} $ from $Cat(y_{r})$, the unlabelled data samples  $ \{ \bm{x_{u}^{(1)}}, \dots, \bm{x_{u}^{(m)}} \}$ from $p_{data}$ and the labelled data samples  $ \{ \bm{x_{l}^{(1)}}, \dots, \bm{x_{l}^{(m)}} \}$ from $p_{ldata}$. Here, $m$ is the minibatch size.}
    
    \STATE {Update the discriminator $S$ by ascending its stochastic gradient:
        \[
            \nabla_{\theta_{s}} \frac{1}{m} \sum_{i=1}^m \left[\bm{{S_{loss}}}^{(i)}\right].
        \]}   
        
    \STATE {Update the discriminator $L$ by ascending its stochastic gradient:
        \[
            \nabla_{\theta_{l}} \frac{1}{m} \sum_{i=1}^m \left[\bm{{L_{loss}}}^{(i)}\right].
        \]}   
  \ENDFOR
   
    \STATE {Repeat step [3].}
    
    \STATE {Update the Encoder $E$, Decoder $D$, and Classifier $C$ by descending its stochastic gradient:
        \[
            \nabla_{\theta_{e},\theta_{d},\theta_{c}} \frac{1}{m} \sum_{i=1}^m \left[\bm{{EDC_{loss}}}^{(i)} \right].
        \]}
     \ENDFOR

% \algstore{myalg}
\end{algorithmic}
\end{algorithm}








==> results_old.tex <==
For comparing the result of GGAN model, we have trained unsupervised and supervised BigGAN model on S09 dataset. For GGAN model, we need to validate two tasks, one is the representation learning, and another one is the sample generation quality. During the validation of representation learning, we also need to verify whether pre guidance is useful for representation learning or not. We expect the GGAN model to outperform unsupervised BigGAN in terms of representation learning and sample generation. We also expect the sample generation quality to be similar or nearby to the supervised BigGAN. 


% Before implementing the GGAN model, we have trained unsupervised and supervised BigGAN model on S09 dataset to understand their behaviour as well as for a comparison with GGAN. We had a clear intention to understand whether the representation learned by GGAN is better than any powerful unsupervised GAN, and our GGAN should perform better than any  GAN or near to any supervised GAN. 


\subsection{Unsupervised and Supervised BigGAN}

For unsupervised BigGAN model, we achieved an IS score of 6.17±.2 and an FID score of 24.72 where we received IS score of 7.33±.01 and FID score of 24.40 ± .5 for the supervised BigGAN. Due to having the access to all label information, Supervised BigGAN performed better than the unsupervised BigGAN. But the performance of both networks is better than any other research works showed in the table \ref{tab:my-table}. 


% We have used BigGAN Architecture for the generation of the audio log-magnitude spectrogram for the s09 dataset. For unsupervised BigGAN, we achieved an IS score of 6.17±.2 and an FID score of 24.72 where we received IS score of 7.33±.01 and FID score of 24.40 ± .5 for the supervised setting. As usual, Supervised BigGAN performed better than the unsupervised BigGAN. But the performance of both networks is better than any other research works showed in the table \ref{tab:my-table}. 

\noindent Though we have achieved state of the art sample generation result with the unsupervised BigGAN architecture, we found inconsistency in the latent space.


When we did linear interpolation between two random points in the latent space like the DCGAN paper \cite{radford2015}, we found a smooth transition in the generated spectrogram space but after converting them to the audio, we found the transaction non-smooth. 
\noindent In figure \ref{fig:fig1}, we can observe the generated spectrogram by the generator where the latent input vectors were the result of the linear interpolation between two random latent points. For the first latent point (most left in the figure), the generator has created spectrogram for digit 2 with a male voice, and for the other point (most right in the figure), it has created digit 2 with a female voice. In between are the spectrograms for the interpolated latent vectors. From left to right, we can see a smooth transition between the spectrograms, but when we converted it to the audio form, after the first sample digit 2 with the male voice, we got digit 8 with a new male and female voice. Then there is the digit 2 with the desired female voice. In this example, the digit was the same for two samples (most left and right in the figure), but the voice was changed from male to female. In the audio space, we have noticed the smooth transition for the speaker's voice, but for the digit, we found 8 in between, which is unexpected and shows that the generator was unable to disentangle the information of the digit category properly. 



% In figure \ref{fig:fig2}, we have also noticed the same problem in the interpolation between male voice digit 8 to male voice digit 0. From this, we can understand that the generator was not able to disentangle the major property of the dataset, which is a problem later task such as data augmentation and representation learning. This problem was not found in the supervised BigGAN.      


\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=\textwidth]{images/1.png}}
    \caption{ Generated Spectrogram from the interpolation of the latent space from the male sound of digit 2 to the female sound of digit 2 (left to right). }
    \label{fig:fig1}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=\textwidth]{images/2.png}}
    \caption{ Generated Spectrogram from the interpolation of the latent space from the male sound of digit 8 to the male sound of digit 0 (left to right). }
    \label{fig:fig2}
\end{figure*}


For learning the representation for the real data samples, we implemented the strategy from the Adversarially learned inference paper \cite{dumoulin2016adversarially} and trained a feature extraction layer top of the trained discriminator network. To evaluate the representation, we have trained a classifier for the digit recognition with a fewer label such as 1 to 5 percent and table \ref{tab:my-table2} show us the result.  


% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{table}
\centering
\caption{Comparison of the performance of the audio generation for different research works}
\label{tab:my-table}
\begin{tabular}{|l|l|l|}\hline
\textbf{Model Name} & \textbf{IS Score} & \textbf{FID Score} \\ \hline
Real (Train) & 9.18 ± 0.04 & - \\ \hline
Real (Test) & 8.01 ± 0.24 &  -\\ \hline
TiFGAN & 5.97 & 26.7 \\ \hline
WaveGAN & 4.67 ± 0.01 &  -\\ \hline
SpecGAN & 6.03 ± 0.04 &  -\\ \hline
Supervised BigGAN & 7.33±.01 & 24.40 ± .5  \\ \hline
Unsupervised BigGAN & 6.17±.2 & 24.72±.05 \\ \hline
GGAN & 7.24±.05 & 25.75±.1 \\ \hline
\end{tabular}
\end{table}


\subsection{GuidedGAN (GGAN)}

\noindent We have implemented our GGAN model with the S09 dataset and achieved IS score of 7.24±.05  and FID score of 25.75±.1 for audio samples using the guidance from 5 percent label data, which is almost near to the performance of the fully supervised Biggan model and far more better than unsupervised BigGAN. 

\begin{figure*}[h]
    \centering
    \frame{\includegraphics[width=\textwidth]{audios.png}}
    \caption{ Generated log-magnitude spectrograms for different conditions. The rows represents different samples generated for different latent space for the given condition (digits)}
    \label{fig:fig3}
\end{figure*}


\noindent GGAN model not only performed Superior in terms of generation but also performed state of the art in the representation learning. With 5 percent label data, we have achieved approximately the test classification accuracy of 95. If we compare the result from table \ref{tab:my-table2} for GGAN and Unsupervised GAN, we can see that for a similar number of the labeled dataset, we have achieved better results with the GGAN. At the same time, it also performed better at generation. 

\begin{table}
\centering
\caption{Comparison of the test accuracy for unsupervised GAN and GGAN}
\label{tab:my-table2}\\
\begin{tabular}{|l|l|l|}\hline
\textbf{Training Data Size} & \textbf{Unsupervised GAN} & \textbf{GGAN} \\ \hline
1\% & 73 ± 1.02 &  84 ± 2.24\\ \hline
2\%  & 75 ± 0.41 &  85 ± 1.24\\ \hline
3\%  & 78 ± 0.07 & 88 ±.1 \\ \hline
4\%  & 80 ± 0.01 &  92 ± 0.5 \\ \hline
5\%  & 80 ± 1.72 &  94 ± 1.2\\ \hline
\end{tabular}
\end{table}

\noindent We have also use TSNE to visualize the learned representation space for the test dataset. Figure \ref{fig:fig3} shows the representations, and we can see that the learned representations are easily classifiable.


\begin{figure}[h]
    \centering
    \frame{\includegraphics[width=.8\linewidth]{images/embfinal.png}}
    \caption{ TSNE visualisation of the learned embedding on the test dataset. }
    \label{fig:fig3}
\end{figure}

\noindent For the second experiment, we have achieved generated samples of S09 for males and females for two different conditions. So the guidance of gender has worked successfully from a completely different dataset. We achieved IS score of 6.52 ± .5 and FID score of 26.21 ± .1. Though our GGAN model was not guided for digit categories, it has SOTA performance. 



\noindent Among many minor challenges, the main challenge we faced was related to the generation of the model. There was a severe issue of mode collapse, which we could not fix implementing different techniques in the literature \cite{salimans:2016}. So we got inspiration from the Mode Seeking GAN \cite{Qi05628} work and modified the loss function and created a unique feature loss, which immediately fixed the mode collapse problem. The feature loss calculates the ratio of the difference between the two real samples and two generated samples. The whole model wants to minimise this loss until the value one. If the generator creates very similar or the same sample, then it gets penalised and tries to find more modes.  In the supplement material section, we have provided the detail of the training and the discussion on the behaviour of the losses as these are an essential guideline for reproducing the results or improve the work only.







==> texes/metadaten.tex <==
%%Hier alle Daten einfügen
\newcommand{\autorname}{Kazi Nazmul Haque (u1104280)}

\newcommand{\Program}{Doctor of Philosophy (DPHD)}
\newcommand{\Faculty}{Faculty of Health, Engineering, and Sciences}
\newcommand{\School}{Agricultural, Computation and Environment Science}
\newcommand{\ps}{Dr Rajib Rana}
\newcommand{\as}{Ji Zhang}
\newcommand{\lp}{Lehrperson}
\newcommand{\arbtyp}{}
\newcommand{\titel}{Learning Unsupervised Distangled Representation
From Audio for Transfer Learning.}
\title{\titel}
\author{\autorname}








% Program: 
% Faculty: 
% School: School of Psychology and Counselling
% Area of study: Health Systems and Behaviour
% Principal Supervisor: Assoc. Prof. Sonja March
% Associate Supervisors: Dr. Belinda Goodwin, Prof. Jeff Dunn AO

==> texes/titlepage.tex <==
\begin{titlepage}
\vspace*{4cm}
\begin{tabu} to \textwidth {X[c]}
	\toprule
	\toprule[2pt]
	\huge{\textsc{\titel}}\\
	\Large{\textsc{\arbtyp}}\\
	\bottomrule[2pt]
	\bottomrule
\end{tabu}
\\[3cm]
\centering{
\textsc{\Large \autorname}
}
\\[3cm]
\begin{tabu} {>{\itshape}X[r] X[1.5]}
Program & \Program\\
Faculty & \Faculty\\
School & \School\\
Principle Supervisor & \ps\\
Associate Supervisors & \as \\
\end{tabu}
\vfill
\includegraphics[width=3cm]{res/usq.jpg}

\end{titlepage}

